GPT Understands, Too

Prompting a pretrained language model with natural language patterns has been proved effective for natural language understanding (NLU). However, our preliminary study reveals that manual discrete prompts often lead to unstable performance -- e.g., changing a single word in the prompt might result in substantial performance drop. We propose a novel method P-Tuning that employs trainable continuous prompt embeddings in concatenation with discrete prompts. Empirically, P-Tuning not only stabilizes training by minimizing the gap between various discrete prompts, but also improves performance by a sizeable margin on a wide range of NLU tasks including LAMA and SuperGLUE. P-Tuning is generally effective for both frozen and tuned language models, under both the fully-supervised and few-shot settings.

==> 3_problem.tex <==
\section{Problem Setup}

Language models could grasp knowledge during pre-training from scratch, but it is difficult to evaluate. Although super large language models keep breaking records in wide range of downstream tasks, the fact that it requires sufficient fine-tuning confuses the knowledge learned during the pre-training with what is learned during the fine-tuning, and thus fails to demonstrate what language models really learn much knowledge from pre-training.

To evaluate the authentic knowledge language models acquired from pre-training, in this work we propose two proxy tasks that require no or minimum efforts for fine-tuning: knowledge probing and few-shot learning.

\subsection{Knowledge Probing}
Narrowly speaking, the knowledge usually refers to the world knowledge in the knowledge base. The knowledge probing, or mentioned as fact retrieval, is about evaluating how much real-world knowledge has language models gained from pre-training. The LAMA dataset evaluates it with cloze tests created from triples selected in the knowledge bases. For example, we will transform the triple (Dante, born-in, Florence) into a cloze sentence with handcraft prompt ``Dante was born in [MASK].", and then we ask language models to perform zero-shot inference.

\subsection{Few-shot Learning}


In addition to world knowledge, it has been proved that language models can also provide prior knowledge for specific downstream tasks (denoted as prior-task knowledge).
The commonly-used few-shot learning tasks are considered.
By using prompts to reformulate inputs into cloze-style phrases and equally transform the discriminative few-shot tasks into masked language model tasks, they are able to make use of the linguistic knowledge within language model.
For example, a sentiment analysis task (``Best movie ever!'', +1) would be transformed into masked language model tasks (``Best movie ever! It was [MASK].''), where predicting ``[MASK]'' to be ``great'' equals ``+1'' labeling.
In this way, the inherent linguistic knowledge would guide the prediction of masked token, which further help few-shot task prediction.


Similar to knowledge probing, the prompt-based prediction can be directly performed over given pretrained language models in a zero-shot manner.
Particularly, since different tasks are independent, it is also applicable for few-shot learning to fine-tune on given pretrained language models, making them more adaptive for specific tasks.





==> tables/ablation_study.tex <==
\begin{table}
    \scriptsize
    \centering
    %\vspace{-9mm}
    \begin{threeparttable}
    \begin{tabular}{c|c|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}}
        \toprule[1pt]
        \multirow{2}{*}{Models} & \multirow{2}{*}{\makecell[c]{Prompt\\Encoder}} & BoolQ & RTE & WSC\\ 
         &  & (Acc.) & (Acc.) & (Acc.) \\ 
         \hline
        \multirow{2}{*}{albert}
        & LSTM & 78.53 & 76.9 & 77.88 \\
        & MLP   & 76.15 & 72.56 & 82.69\\
        & Emb   & 76.61 & 71.11 & 78.84 \\
        %\midrule[1pt]
        % \multirow{2}{*}{deberta}
        %& LSTM & 80.70 & 76.90 & 86.53 \\
        %& MLP & 81.28 & 80.51 & 85.57\\
        %& Emb & 80.79 & 81.22 & 78.84 \\
    \bottomrule[1pt]
    \end{tabular}
    \end{threeparttable}
    \caption{Ablation analysis for prompt encoder with albert-xxlarge-v2. For each experiment, the checkpoint is selected according to performance on $\mathcal{D}_{dev32}$, and report the performance on SuperGLUE dev set.}
    \label{tab:superglue-ablation}
    \vspace{-4mm}
\end{table}

==> tables/few_superglue.tex <==
\begin{table*}[tb]
\scriptsize
\centering
\scalebox{1.0}{
\begin{threeparttable}
    \begin{tabular}{c|c|l|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}}
    \toprule[1pt]
    Pretrained & Dev 
        & \multirow{2}{*}{Method} 
        & BoolQ 
        & \multicolumn{2}{c|}{CB} 
        & WiC 
        & RTE 
        & \multicolumn{2}{c|}{MultiRC}  
        & WSC 
        & COPA \\ 
    model & size &
    & (Acc.) 
    & (Acc.) 
    & (F1) 
    & (Acc.) 
    & (Acc.) 
    & (EM) 
    & (F1a) 
    & (Acc.) 
    & (Acc.) 
    \\ \hline
    \multirow{3}{*}{albert} & \multirow{3}{*}{32} 
    & PET$^*$ 
        & 75.17
        & 85.71
        & 79.74
        & 54.39
        & 71.84
        & 32.0
        & 75.62
        & 79.81
        & 87.0 \\
        %& 73.2\tiny{$\pm$3.1} 
        %& 82.9\tiny{$\pm$4.3} 
        %& 74.8\tiny{$\pm$9.2}  
        %& 51.8\tiny{$\pm$2.7}  
        %& 62.1\tiny{$\pm$5.3}  
        %& 33.6\tiny{$\pm$3.2} 
        %& 74.5\tiny{$\pm$1.2}   
        %& 79.8\tiny{$\pm$3.5}  
        %& 80.5\tiny{$\pm$5.1} \\
    % & & PET best$^\dagger$ & 75.1  & 86.9 & 83.5  & 52.6  & 65.7  & 35.2  & 75.0  & 80.4  & 83.3 \\ 
    & & P-tuning $^*$
        & 78.53 \tiny{\color{red}{(+3.36)}}
        & 89.29 \tiny{\color{red}{(+3.58)}}
        & 86.79 \tiny{\color{red}{(+7.05)}}
        & 52.98 \tiny{\color{blue}{(-1.41)}}
        & 76.9 \tiny{\color{red}{(+5.06)}}
        & 37.04 \tiny{\color{red}{(+5.04)}}
        & 75.5 \tiny{\color{blue}{(-0.12)}}
        & 82.69 \tiny{\color{red}{(+2.88)}}
        & 87.0 \tiny{\color{red}{(+0.0)}} \\
        %& 77.8 \tiny{\color{red}{(+4.6)}}
        %& 92.9 \tiny{\color{red}{(+10.0)}}
        %& 92.3 \tiny{\color{red}{(+17.5)}}
        %& 56.3 \tiny{\color{red}{(+4.5)}}
        %& 76.5 \tiny{\color{red}{(+14.4)}}
        %& 36.1 \tiny{\color{red}{(+2.5)}}
        %& 75.0 \tiny{\color{red}{(+0.5)}}
        %& 84.6 \tiny{\color{red}{(+4.8)}}
        %& 87.0 \tiny{\color{red}{(+6.5)}}\\ 
    
    \hline%\midrule[1pt]
    \multirow{4}{*}{albert} & \multirow{4}{*}{Full}
    & GPT-3 $\dagger$
        & 77.5 
        & 82.1 
        & 57.2 
        & 55.3 
        & 72.9 
        & 32.5 
        & 74.8 
        & 75.0 
        & 92.0 \\
    & & PET$^\ddagger$ $\dagger$
        & 79.4 
        & 85.1 
        & 59.4 
        & 52.4 
        & 69.8 
        & 37.9 
        & 77.3 
        & 80.1 
        & 95.0 \\
    & & iPET$^\mathsection$ $\dagger$
        & 80.6 
        & 92.9 
        & 92.4 
        & 52.2 
        & 74.0 
        & 33.0 
        & 74.0 
        & -    
        & - \\ 
    % & & ADAPET$\dagger$
    %    & 80.3
    %    & 89.3
    %    & 86.8
    %    & 54.4
    %    & 76.5
    %    & 39.2
    %    & 80.1
    %    & 81.7
    %    & 89.0 \\ 
    % \midrule[1pt]
    % \multirow{3}{*}{deberta} & \multirow{3}{*}{32} 
    % & PET$^*$    
    %    & 80.73
    %    & 85.71
    %    & 80.49
    %    & 58.46
    %    & 78.70
    %    & 43.75
    %    & 79.17
    %    & 85.57
    %    & 80.0 \\
    %& & P-tuning $^*$
    %    & 81.28 \tiny{\color{red}{(+0.55)}}
    %    & 87.5 \tiny{\color{red}{(+1.79)}}
    %    & 81.74 \tiny{\color{red}{(+1.25)}}
    %    & 53.45 \tiny{\color{blue}{(-5.01)}}
    %    & 80.51 \tiny{\color{red}{(+1.81)}}
    %    & 39.03 \tiny{\color{blue}{(-4.72)}}
    %    & 76.25 \tiny{\color{blue}{(-2.92)}}
    %    & 85.57 \tiny{\color{red}{(+0.0)}}
    %    & 77.0 \tiny{\color{blue}{(-3.0)}}
    %    \\
    \bottomrule[1pt]
    \end{tabular}
    \begin{tablenotes}
        \item[*] \small Experiments are conducted under the new few-shot setting. Checkpoints \& hyper-params are selected according to the performance of $\mathcal{D}_{dev32}$.
        % \item[$\dagger$] \small We report the best performed prompt selected on \textit{full} dev dataset among all candidate prompts.
        \item[$\dagger$] \small Results are reported by corresponding papers.
        \item[$\ddagger$] \small With additional ensemble and distillation.
        \item[$\mathsection$] \small With additional data augmentation, ensemble, distillation and self-training.
    \end{tablenotes}
    \end{threeparttable}
    }
    \vspace{-5pt}
    \caption{Few-shot learning performance on SuperGLUE dev. 
    Previous few-shot learning approaches use the original full dev set $\mathcal{D}_{dev}$ for validation, which does not make sense. 
    We construct a new dev set $\mathcal{D}_{dev32}$ with 32 unused samples from original training set. 
    Under fair comparison, \solution significantly outperforms PET($\mathcal{D}_{dev32}$) and PET best($\mathcal{D}_{dev32}$) on all tasks. 
    More interestingly, \solution even outperforms GPT-3, PET($full$) and iPET($full$) on 4 out of 7 tasks. 
    Subscripts in red represents the improvements of \solution over PET($\mathcal{D}_{dev32}$).}
    \label{tab:fewshot:ultimate}
    \vspace{-4mm}
\end{table*}
